QScale: Probabilistic Chained Consensus for Moderate-Scale Systems

Existing distributed ledger protocols either incur a high communication complexity and are thus suited to systems with a small number of processes (e.g., PBFT), or rely on committee-sampling-based approaches that only work for a very large number of processes (e.g., Algorand). Neither of these lines of work is well-suited for moderate-scale distributed ledgers ranging from a few hundred to a thousand processes, which are common in production (e.g, Redbelly, Sui). The goal of this work is to design a distributed ledger with sub-linear communication complexity per process, sub-quadratic total communication complexity, and low latency for finalizing a block into the ledger, such that it can be used for moderate-scale systems. We propose QScale, a protocol in which every process incurs only $\widetilde{O}(\kappa \sqrt{n})$ communication complexity per-block in expectation, $\widetilde{O}(n\kappa)$ total communication complexity per-block in expectation, and a best-case latency of $O(\kappa)$ rounds while ensuring safety and liveness with overwhelming probability, with $\kappa$ being a small security parameter.

==> extended_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

In this section, we present concrete probabilities for the safety and liveness guarantees of our protocol.
We also compare our design with fixed-committee designs.

\ignore{
\myparagraph{Synchronous setting.}
We set the parameters as follows:
$n = 500$,
$q = 49$, 
$\prSample = 3/\sqrt{n}$, 
$\prSample = 1.9q/n$, and
$\prProp = 10/n$.
Fig.~\ref{fig:safety-violation} shows the log-scaled probability of a safety violation as a function of~$\kappa$ for three different values of the fault ratio: $f/n = \epsilon \in \{0.2, 0.3, 0.4\}$.
As expected, the probability of a safety violation exponentially decreases as~$\kappa$ increases, with faster decay for lower values of~$\epsilon$.
The results show that even for relatively high fault ratios (e.g., $\epsilon = 0.4$), a moderate value of~$\kappa$ (e.g., $\kappa = 7$) suffices to reduce the probability of a safety violation below $2^{-30}$. 
%This analysis demonstrates that \protocolName provides strong probabilistic safety guarantees while allowing clients to tune the commitment depth~$\kappa$ according to their desired level of confidence.
Besides, Fig.~\ref{fig:liveness} illustrates the probability of committing in $\kappa$ epochs in the best-case scenario, for the same fault ratios $\epsilon \in \{0.2, 0.3, 0.4\}$. 
As~$\kappa$ increases, the probability of committing in $\kappa$ epochs decreases. 

\kartik{what is a practical way of choosing $q$? Should one always set it as 8 log n? or should one think of it as a free parameter?}

\begin{figure}[!t]
    \centering
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[scale=0.46]{figures/500-safety-sync.pdf}
        \caption{Probability of safety violation vs. $\kappa$. 
        % The y-axis shows the logarithm (base 10) of the safety violation probability as a function of the commitment depth~$\kappa$.
        }
        \label{fig:safety-violation}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[scale=0.46]{figures/500-liveness-sync.pdf}
        \caption{Probability of committing in $\kappa$ epochs.}
        \label{fig:liveness}
    \end{subfigure}
    \caption{Evaluation under synchrony with $n=500$.}
    \label{fig:main}
\end{figure}
}

\begin{figure*}[!t]
    \centering
    \includegraphics[scale=0.53]{figures/500-psync.pdf}
    \caption{The probability of safety violation (top) and of committing in $\kappa$ epochs (bottom) with $n=500$.
    The expected sample size is $3q/2$, and 
    $q \in \{2\sqrt{n},3\sqrt{n},4\sqrt{n}\}$.}
    \label{fig:psync:3q}
\end{figure*}

\begin{figure*}[!t]
    \centering
    \includegraphics[scale=0.53]{figures/1000-psync-2-3-4.pdf}
    \caption{The probability of safety violation (top) and of committing in $\kappa$ epochs (bottom) with $n=1000$.
    The expected sample size is $3q/2$, and 
    $q \in \{2\sqrt{n},3\sqrt{n},4\sqrt{n}\}$.}
    \label{fig:psync:1000}
\end{figure*}

\begin{figure*}[!t]
    \centering
    \includegraphics[scale=0.53]{figures/1000-psync-bigger-samples.pdf}
    \caption{The probability of safety violation (top) and of committing in $\kappa$ epochs (bottom) with $n=1000$.
    The expected sample size is $3q/2$, and 
    $q \in \{3.3\sqrt{n},4.9\sqrt{n},5.7\sqrt{n}\}$.}
    \label{fig:psync:1000:similar:to:500}
\end{figure*}

We consider two values for $n$: $500$ and $1000$.
For the first two experiments, we consider three values of $q$: $2\sqrt{n}$, $3\sqrt{n}$, and $4\sqrt{n}$.
The other parameters are as follows:
$\prSample = 1.5q/n$,  
$\prProp = 6/n$, and
$\alpha = 5$.
Fig.~\ref{fig:psync:3q} and Fig.~\ref{fig:psync:1000} show the log-scaled probability of a safety violation under partial synchrony as a function of~$\kappa$ for four different values of the fault ratio: $f/n = \epsilon \in \{0.1, 0.15, 0.2, 0.25\}$.
\ignore{Overall, the behavior of the probability curves is similar to what was observed for synchronous settings, but with worse values.}
%As expected, the probability of a safety violation decreases exponentially as~$\kappa$ increases, with faster decay for lower values of~$\epsilon$.
%As~$\kappa$ increases, the probability of committing in $\kappa$ epochs decreases. 
The results show that the safety violation probability decreases faster with bigger quorums.
Besides, the probability of committing in $\kappa$ epochs gets better with bigger quorums. 

Fig.~\ref{fig:psync:1000} provides stronger safety guarantees than Fig.~\ref{fig:psync:3q}, but achieves a lower probability of committing within $\kappa$ blocks.
To examine when the cases $n = 1000$ and $n = 500$ exhibit similar behavior, we conducted an additional experiment with $n = 1000$, keeping all parameters unchanged except for $q$.
The results, shown in Fig.~\ref{fig:psync:1000:similar:to:500}, indicate that achieving behavior similar to Fig.~\ref{fig:psync:3q} requires larger values of $q$.

Table~\ref{tab:kappa-values} shows the expected number of messages exchanged and the communication bits per epoch, as well as the smallest value of $\kappa$ that ensures the required safety for the three quorum sizes we consider, for two values of $\epsilon$.
We consider transactions of size $250$ bytes and employ BLS multi-signatures.
Although larger values of $q$ increase the likelihood of ensuring safety and timely commitment, they come at the cost of violating the sub-linear per-process communication objective of \protocolName, as shown in the table.

Note that these results consider a network where partitions can happen and the adversary can manipulate message scheduling.
If the network behaves well (synchronous case), or the network adversary is limited (as in~\cite{probft}), the probabilities are much better.
In any case, given an expected $\epsilon$, one decides the target number of bits of security (for ensuring safety) and picks the most appropriate quorum size and expected $\kappa$ (these values can be changed on each epoch).
Then, the protocol will make progress when the fraction of actual failures in the system is small (possibly $\ll \epsilon$), but progress will become less frequent as the fraction of compromised processes increases, depending on the actual $\kappa$ clients use. 


\begin{table*}[!t]
\centering
% \caption{Minimum $\kappa$ values for different $q$ and safety violation probabilities.}
\caption{Communication per epoch and values of $\kappa$ for various target security.}
\label{tab:kappa-values}
\begin{tabular}{@{}c@{\hspace{0.5em}}c@{\hspace{0.5em}}l@{\hspace{0.5em}}l@{\hspace{0.5em}}l@{\hspace{0.75em}}l@{\hspace{0.75em}}l@{\hspace{0.75em}}l@{\hspace{0.75em}}l@{}}
\toprule
\vspace{-0.2em}
         \multirow{2}{*}{\shortstack[c]{Quorum\\ size}}
         & \multirow{2}{*}{\shortstack[c]{A leader's comm.\\per epoch}}
         & \multirow{2}{*}{\shortstack[c]{Total messages/\\ comm. per epoch}} 
         & \multicolumn{3}{c}{Safety $(\epsilon = 0.1)$} & 
         \multicolumn{3}{c}{Safety $(\epsilon = 0.15)$} 
         \\ \cmidrule(lr){4-6} \cmidrule(lr){7-9} 
         & & & $2^{-20}$ & $2^{-30}$ & $2^{-40}$ & $2^{-20}$ & $2^{-30}$ & $2^{-40}$ 
\vspace{-0.2em}
\\ \midrule       
\vspace{-0.2em}
$q = 44$ & $37\,\mathrm{kb}$ & $13640$ / $3740\,\mathrm{kb}$ & $\kappa = 3$ & $\kappa = 4$ & $\kappa = 5$ & $\kappa=4$ & $\kappa=5$ & $\kappa=6$

\\ \midrule
\vspace{-0.2em}
$q = 67$ & $39\,\mathrm{kb}$ & $13678$ / $3742\,\mathrm{kb}$ & $\kappa = 2$ & $\kappa = 3$ & $\kappa = 4$ & $\kappa=3$ & $\kappa=4$ & $\kappa=5$

\\ \midrule
\vspace{-0.2em}
$q = 89$ & $41\,\mathrm{kb}$ & $13715$  / $3745\,\mathrm{kb}$ & $\kappa = 2$ & $\kappa = 3$ & $\kappa = 4$ & $\kappa=2$ & $\kappa=3$ & $\kappa=4$

\\ \bottomrule
\end{tabular}
\end{table*}

\ignore{
\myparagraph{Comparing with fixed committee designs.} 
We also compared \protocolName with an alternative design in which processes run the protocol with a static committee of size $c$ instead of selecting different samples of $O(\sqrt{n})$ for each step.
This design has $O(c)$ per-process message and communication complexities.
The results, fully explained in Appendix~\ref{app:static:commitee}, show that these committees have to contain 65\% of the processes to have a safety violation probability smaller than $2^{-30}$ when $n=500$ and $f=200$.
In this setting, our protocol requires only $65\%$ of the communication required if PBFT were run in this committee to achieve similar security under synchrony.
For larger values of $n$, $c/n$ decreases, still requiring each process to send significantly more messages than in our protocol. 
}


\ignore{
\section{Evaluation under Synchrony}
\label{sec:evaluation:sync}

In this section, we present concrete numbers for the probabilities of safety and liveness guarantees of our protocol under synchrony.  

% \myparagraph{Setting.}
We set the parameters as follows:
$n = 500$,
$q = 49$, 
$\prSample = 3/\sqrt{n}$, 
$\prSample = 1.9q/n$, and
$\prProp = 10/n$.
Fig.~\ref{fig:safety-violation} shows the log-scaled probability of a safety violation as a function of~$\kappa$ for three different values of the fault ratio: $f/n = \epsilon \in \{0.2, 0.3, 0.4\}$.
As expected, the probability of a safety violation exponentially decreases as~$\kappa$ increases, with faster decay for lower values of~$\epsilon$.
The results show that even for relatively high fault ratios (e.g., $\epsilon = 0.4$), a moderate value of~$\kappa$ (e.g., $\kappa = 7$) suffices to reduce the probability of a safety violation below $2^{-30}$. 
%This analysis demonstrates that \protocolName provides strong probabilistic safety guarantees while allowing clients to tune the commitment depth~$\kappa$ according to their desired level of confidence.
Besides, Fig.~\ref{fig:liveness} illustrates the probability of committing in $\kappa$ epochs in the best-case scenario, for the same fault ratios $\epsilon \in \{0.2, 0.3, 0.4\}$. 
As~$\kappa$ increases, the probability of committing in $\kappa$ epochs decreases. 

\kartik{what is a practical way of choosing $q$? Should one always set it as 8 log n? or should one think of it as a free parameter?}

\begin{figure}[hbt]
    \centering
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[scale=0.46]{figures/500-safety-sync.pdf}
        \caption{Probability of safety violation vs. $\kappa$. 
        % The y-axis shows the logarithm (base 10) of the safety violation probability as a function of the commitment depth~$\kappa$.
        }
        \label{fig:safety-violation}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[scale=0.46]{figures/500-liveness-sync.pdf}
        \caption{Probability of committing in $\kappa$ epochs.}
        \label{fig:liveness}
    \end{subfigure}
    \caption{Evaluation under synchrony with $n=500$.}
    \label{fig:main}
\end{figure}


% \section{Effect of Varying $q$ on Protocol Behavior}
% \label{sec:effect:of:q}

% In this section, we elaborate on the effect of varying $q$ on \protocolName.
% Since \protocolName employs multi-signatures, increasing $q$ from $a$ to $b$ adds only $(b-a)\times n$ bits to the communication complexity of each epoch. \kartik{this is not entirely true, correct. the leader does need to receive all of these signature shares?}
% In contrast, without multi-signatures, the same increase in $q$ would add $(b-a)\times n$ individual signatures, thereby directly increasing the communication cost.
% These results are reflected in Table~\ref{tab:comparision}, which shows that different values of $q$ do not significantly change the communication cost.
% On the other hand, increasing $q$ improves the probability of ensuring safety and committing in $\kappa$ epochs. 
% Fig.~\ref{fig:q} complements this result by showing the probability of safety violation and of committing in $\kappa$ epochs, under partial synchrony, when $n=500$, $\prSample=3/\sqrt{n}$, $\prProp = 6/n$, $\kappa=5$, $f/n=\epsilon=0.1$, and $\prSample=1.45q/n$.
% This naturally raises the question: if increasing $q$ does not significantly increase communication complexity, why not simply increase $q$ to the maximum possible value to maximize the probability of safety and commitment within $\kappa$ epochs?

% To answer this question, recall that one of our main goals in designing \protocolName is to achieve \emph{sub-linear communication per process}. 
% To this end, we set the protocol parameters so that, in each epoch and under best-case scenarios, the leader receives at least $q$ messages required to certify the block proposed in the previous epoch. 
% However, when $q$ is large, the leader's communication complexity is no longer sub-linear.
% In summary, while larger values of $q$ increase the likelihood of ensuring safety and timely commitment, they come at the cost of violating the sub-linear per-process communication objective of \protocolName.

% \begin{figure}[!t]
%     \centering
%     \begin{subfigure}[t]{0.49\textwidth}
%         \centering
%         \includegraphics[scale=0.46]{figures/safety-violation-q.pdf}
%         % \caption{Probability of a safety violation vs. $q$.}
%         % \label{fig:safety:violation:q}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.49\textwidth}
%         \centering
%         \includegraphics[scale=0.46]{figures/liveness-q.pdf}
%         % \caption{Probability of committing in $\kappa$ epochs vs. $q$.}
%         % \label{fig:liveness:q}
%     \end{subfigure}
%     \caption{Effect of varying $q$ on the probability of safety violation (left) and of committing in $\kappa$ epochs (right).}
%     \label{fig:q}
% \end{figure}
}
